From geodesic flow to wave dynamics on hyperbolic surfaces

We study the geodesic flow on the unit cotangent bundle $M=S^{*}\mathcal{N}$ of a closed hyperbolic surface $\mathcal{N}$, using the representation theory of $SL_{2}(\mathbb{R})$. We construct explicit $X$-adapted Hilbert spaces, obtained by completing propagated dense domains of $L^{2}(M)$, which are tailored to the spectral analysis of the geodesic generator $X$. In these spaces, $X$ becomes a normal operator with discrete spectrum, except at the threshold $\mu=1/4$, where Jordan blocks of size two may occur. In this Hilbert model, the propagator $e^{tX}$ factorizes into a damped harmonic oscillator with eigenvalues $e^{-t(n+1/2)}$, $n\in\mathbb{N}$, and a transverse part involving the shifted wave group $e^{\pm it\sqrt{\Delta-1/4}}$ on $\mathcal{N}$, together with the holomorphic and anti-holomorphic discrete series. The model clarifies two classical links between geodesic dynamics and the Laplace spectrum. Comparing the spectral trace of the propagator in the $X$-adapted Hilbert model with the Atiyah--Bott--Guillemin flat trace gives a dynamical form of the Selberg trace formula: closed geodesics arise from the flat trace, while the spectral side comes from the explicit $SL_{2}(\mathbb{R})$-decomposition. The same factorization also explains the large-time structure of spherical mean operators on $\mathcal{N}$: after the natural $e^{t/2}$-renormalization and the removal of a finite-rank low-energy part, the shifted wave equation on $\mathcal{N}$ emerges as the leading effective dynamics. Thus the construction provides an explicit Hilbert-space structure relating classical geodesic dynamics, Ruelle resonances, and the spectral theory of the surface.

==> figures/default <==
#FIG 3.2  Produced by xfig version 3.2.8b
Landscape
Center
Metric
A4
100.00
Single
-2
1200 2
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 5400 4950 5400 1800
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2700 3150 8100 3150
4 0 0 50 -1 0 12 0.0000 2 180 315 8055 3420 $k$\001
4 0 0 50 -1 0 12 0.0000 2 180 540 5490 1890 $\\mu$\001

